The Rule of Three: Abstractive Text Summarization in Three Bullet Points

Neural network-based approaches have become widespread for abstractive text summarization. Though previously proposed models for abstractive text summarization addressed the problem of repetition of the same contents in the summary, they did not explicitly consider its information structure. One of the reasons these previous models failed to account for information structure in the generated summary is that standard datasets include summaries of variable lengths, resulting in problems in analyzing information flow, specifically, the manner in which the first sentence is related to the following sentences. Therefore, we use a dataset containing summaries with only three bullet points, and propose a neural network-based abstractive summarization model that considers the information structures of the generated summaries. Our experimental results show that the information structure of a summary can be controlled, thus improving the performance of the overall summarization.

==> pair_result.tex <==
% Each results
\begin{table*}[t]
  \center
  \begin{subtable}{\textwidth}
  \scalebox{0.95}{
  \begin{tabular}{c|rrr|rrr|rrr|rrr}
    \hline
    &\multicolumn{3}{c|}{Coverage} & \multicolumn{3}{c|}{Parallel\_model} 
    & \multicolumn{3}{c|}{Sequence\_model} & \multicolumn{3}{c}{Proposed} \\ \hline 
          %&\multicolumn{3}{c|}{ROUGE} &\multicolumn{3}{c|}{ROUGE} &\multicolumn{3}{c|}{ROUGE} &\multicolumn{3}{c}{ROUGE} \\
          % &1 & 2 & L & 1 & 2 & L & 1 & 2 & L & 1 & 2 & L \\ \hline
          & \multicolumn{1}{c}{R-1} & \multicolumn{1}{c}{R-2} & \multicolumn{1}{c|}{R-L} & 
           \multicolumn{1}{c}{R-1} & \multicolumn{1}{c}{R-2} & \multicolumn{1}{c|}{R-L} & 
           \multicolumn{1}{c}{R-1} & \multicolumn{1}{c}{R-2} & \multicolumn{1}{c|}{R-L} & 
           \multicolumn{1}{c}{R-1} & \multicolumn{1}{c}{R-2} & \multicolumn{1}{c}{R-L} \\ \hline
                1st & 47.04 & 27.12 & 34.01 & 48.01 & 27.86 & 34.54 & 47.81 & 27.27 & 33.95       & {\bf 48.90} & {\bf 28.32} & {\bf 35.12}\\
                2nd & 28.99 & 9.84 & 18.71 & 29.27 & 9.84 & 18.78 & {\bf 29.59} & 10.18 & 19.10         & 29.50 & {\bf 10.38} & {\bf 19.18}\\
                3rd & 26.79 & 8.05 & 17.87 & 27.14 & 8.26 & 18.19 & {\bf 27.58} & {\bf 8.59} & {\bf 18.42}          & 26.85 & 7.67 & 17.91 \\
                Ave & 34.27 & 15.00 & 23.53 & 34.81 & 15.32 & 23.83 & 35.00 & 15.35 & 23.83 & {\bf 35.08} & {\bf 15.46} & {\bf 24.07}\\
    \hline
  \end{tabular}
  }
  \subcaption{Evaluation results in all test data.}
  \label{each_all}
  \end{subtable}


  \center
  \begin{subtable}{\textwidth}
  \scalebox{0.95}{
  \begin{tabular}{c|rrr|rrr|rrr|rrr}
    \hline
    &\multicolumn{3}{c|}{Coverage} & \multicolumn{3}{c|}{Parallel\_model} 
    & \multicolumn{3}{c|}{Sequence\_model} & \multicolumn{3}{c}{Proposed} \\ \hline 
          %A&\multicolumn{3}{c|}{ROUGE} &\multicolumn{3}{c|}{ROUGE} &\multicolumn{3}{c|}{ROUGE} &\multicolumn{3}{c}{ROUGE} \\
          % &1 & 2 & L & 1 & 2 & L & 1 & 2 & L & 1 & 2 & L \\ \hline
          & \multicolumn{1}{c}{R-1} & \multicolumn{1}{c}{R-2} & \multicolumn{1}{c|}{R-L} & 
           \multicolumn{1}{c}{R-1} & \multicolumn{1}{c}{R-2} & \multicolumn{1}{c|}{R-L} & 
           \multicolumn{1}{c}{R-1} & \multicolumn{1}{c}{R-2} & \multicolumn{1}{c|}{R-L} & 
           \multicolumn{1}{c}{R-1} & \multicolumn{1}{c}{R-2} & \multicolumn{1}{c}{R-L} \\ \hline
                1st & 46.88 & 25.93 & 33.10 & 47.27 & 25.86 & 33.42 & 47.56 & 25.61 & 33.09 & {\bf 48.62} & {\bf 28.18} & {\bf 34.76}\\
                2nd & 28.94 & 8.98 & 18.45 & {\bf 30.20} & 10.17 & 19.38 & 30.12 & 9.90 & 19.17   & 29.68 & {\bf 10.67} & {\bf 19.45}\\
                3rd & 28.94 & 8.57 & 19.45 & 29.41 & {\bf 9.12} & {\bf 20.10} & {\bf 29.50} & 8.63 & 19.86    & 26.38 & 7.51 & 17.64 \\
                Ave & 34.92 & 14.49 & 23.66 & 35.63 & 15.05 & {\bf 24.30} & {\bf 35.72} & 14.72 & 24.04 & 34.89 & {\bf 15.45} & 23.95\\
    \hline
  \end{tabular}
  }
  \subcaption{Evaluation results in \textit{parallel} test data.}
  \label{each_seq}
  \end{subtable}

  \center
  \begin{subtable}{\textwidth}
  \scalebox{0.95}{
  \begin{tabular}{c|rrr|rrr|rrr|rrr}
    \hline
    &\multicolumn{3}{c|}{Coverage} & \multicolumn{3}{c|}{Parallel\_model} 
    & \multicolumn{3}{c|}{Sequence\_model} & \multicolumn{3}{c}{Proposed} \\ \hline 
          %&\multicolumn{3}{c|}{ROUGE} &\multicolumn{3}{c|}{ROUGE} &\multicolumn{3}{c|}{ROUGE} &\multicolumn{3}{c}{ROUGE} \\
          % &1 & 2 & L & 1 & 2 & L & 1 & 2 & L & 1 & 2 & L \\ \hline
          & \multicolumn{1}{c}{R-1} & \multicolumn{1}{c}{R-2} & \multicolumn{1}{c|}{R-L} & 
           \multicolumn{1}{c}{R-1} & \multicolumn{1}{c}{R-2} & \multicolumn{1}{c|}{R-L} & 
           \multicolumn{1}{c}{R-1} & \multicolumn{1}{c}{R-2} & \multicolumn{1}{c|}{R-L} & 
           \multicolumn{1}{c}{R-1} & \multicolumn{1}{c}{R-2} & \multicolumn{1}{c}{R-L} \\ \hline
                1st & 47.10 & 27.56 & 34.35 & 48.28 & {\bf 28.60} & 34.95 & 47.90 & 27.88 & 34.28 & {\bf 49.00} & 28.37 & {\bf 35.25}\\
                2nd & 29.01 & 10.16 & 18.81 & 28.92 & 9.72 & 18.56 & 29.40 & {\bf 10.28} & {\bf 19.08}  & {\bf 29.43} & 10.27 & {\bf 19.08}\\
                3rd & 25.99 & 7.85 & 17.29 & 26.30 & 7.94 & 17.48 & 26.87 & {\bf 8.58} & 17.89    & {\bf 27.02} & 7.73 & {\bf 18.00} \\
                Ave & 34.03 & 15.19 & 23.48 & 34.50 & 15.42 & 23.66 & 34.73 & {\bf 15.58} & 23.75 & {\bf 35.15} & 15.46 & {\bf 24.11}\\
    \hline
  \end{tabular}
  }
  \subcaption{Evaluation results in \textit{sequence} test data.}
  \label{each_par}
  \end{subtable}

  \caption{Evaluation results for each sentence.
    The scores in the row of `1st' are computed between the first sentence of the system summary and the sentence of the oracle summary.
    The rows of `2nd' and `3rd' are worked out in the same process. 
    The row of `ave' is the average scores of `1st', `2nd' and `3rd'.
  }
  \label{each_description}
\end{table*}

